Vision-Based Autonomous UAV Navigation and Landing for Urban Search and Rescue

Unmanned Aerial Vehicles (UAVs) equipped with bioradars are a life-saving technology that can enable identification of survivors under collapsed buildings in the aftermath of natural disasters such as earthquakes or gas explosions. However, these UAVs have to be able to autonomously navigate in disaster struck environments and land on debris piles in order to accurately locate the survivors. This problem is extremely challenging as pre-existing maps cannot be leveraged for navigation due to structural changes that may have occurred. Furthermore, existing landing site detection algorithms are not suitable to identify safe landing regions on debris piles. In this work, we present a computationally efficient system for autonomous UAV navigation and landing that does not require any prior knowledge about the environment. We propose a novel landing site detection algorithm that computes costmaps based on several hazard factors including terrain flatness, steepness, depth accuracy, and energy consumption information. We also introduce a first-of-a-kind synthetic dataset of over 1.2 million images of collapsed buildings with groundtruth depth, surface normals, semantics and camera pose information. We demonstrate the efficacy of our system using experiments from a city scale hyperrealistic simulation environment and in real-world scenarios with collapsed buildings.

==> sections/experiments.tex <==
\section{Experimental Setups and Hyperparameters}
\label{sec:experiments}

We evaluate our system extensively in both simulated and real-world scenarios with collapsed buildings. We created a small city-scale simulation environment using the Unreal Engine consisting of collapsed buildings, damaged roads, debris and rubble piles, overturned cars, uprooted trees and several other features resembling a catastrophe struck environment. While, for real-world evaluations, we exhaustively performed experiments at the TCRH Training Center for Rescue in Germany, spanning an area of 60,000 square meters and consisting of scenarios with earthquake and fire damage. \figref{fig:compare_envmt} shows example scenes from both these environments.

\begin{figure}
\centering
\setlength{\tabcolsep}{0.45cm}
\begin{tabular}{p{4cm} p{4cm}}
    \includegraphics[width=\linewidth]{figures/unreal_env.png} & 
    \includegraphics[width=\linewidth]{figures/outdoor_testrun.jpeg} \\
\small{(a) Simulation Environment} & \small{(b) Real-World Outdoor Environment} \\ 
\end{tabular}
  \caption{Evaluation scenarios for our autonomous landing system showing collapsed buildings, overturned vehicles and uprooted trees.}
  \label{fig:compare_envmt}
\end{figure}

\subsection{Hyperrealistic Simulation Environment}

We use the open-source \textit{AirSim} plugin~\cite{airsim2017fsr} with our Unreal Engine environment and ROS as the middleware for our simulation experiments. The simulator considers forces such as drag, friction and gravity in its physics engine, and provides data from various inertial sensors that are required for state estimation. We simulate a downward facing stereo camera mounted to the UAV which provides RGB-D data at $20\hertz$ with a resolution of $640\times480$ pixels, similar to our real-world setup. We clip the groundtruth depth map so that the depth sensor has the range $d_{min} = 0.05\meter$ and $d_{max} = 20.0\meter$. \todo{Write about the dataest being released.} 

\begin{figure}
	\includegraphics[width=\linewidth]{figures/airsim_sample.png}
	\label{fig:airsim_sample}
	\caption{\todo{Sample of the dataset collected using the simulator}}
\end{figure}

We use the same pipeline for state estimation, trajectory planning and landing site detection as in our real-world UAV system. We build an OctoMap at a resolution of $0.5\meter$ and the textured mesh at a resolution of $0.1\meter$. \figref{fig:results}(a) shows an example mesh visualization of a city block created using TSDFs while the UAV followed a lawn-mover surveillance path with a speed of $0.5\meter\per\second$. For the simulation experiments, we set the weights $c_1 = 0.05$, $c_2 = 0.4$, $c_3 = 0.4$ and $c_4 = 0.15$ for the depth accuracy, flatness, steepness and energy consumption costmaps respectively. We consider all the points with scores above $0.72$ in the final decision map as candidate landing sites. We set $c_1 = 0.05$ as the depth map is the groundtruth generated from the simulator. We choose equal weights for flatness and steepness costmaps since they play an equally important role in the landing sites detection. These two costmaps are critical for estimating safe landing sites in collapsed structures as they contain many parts of broken buildings piled on top of each other which appear as several cluttered planes in different orientations. We set the euclidean distance and depth threshold for hierarchical clustering of landing sites to $0.50\meter$ and $0.01\meter$. 
%\href{https://drive.google.com/open?id=1WF47f_vZpaPNYGMWPvEr8Ml7FSnBC6ok}{here}.

\subsection{Real-World Outdoor Environment}

We use the DJI M100 quadrotor equipped with a NVIDIA TX2 embedded computer and a downward facing ZED stereo camera for our real-world experiments. The stereo camera provides RGB-D images with a resolution of $640\times480$ pixels at $20\hertz$. As shown in \figref{fig:overview_system}, we use an EKF to fuse the the raw inertial sensor data with GPS measurements and the pose output obtained from ORB-SLAM2. Similar to the simulation experiments, we use ROS as the middleware on the TX2 which runs all the processes in real-time for state estimation, trajectory planning, landing site detection and bio-radar processing. 

We use an OctoMap resolution of $0.5\meter$ and a textured mesh resolution of $0.1\meter$. \figref{fig:results}(b) shows an example mesh visualization created by the UAV while exploration. Since in the real world, the depthmap generated from stereo images are often noisy, we set $c_1 = 0.15$ in order to account for this factor in the depth accuracy costmap. We set the weights for the flatness, steepness, and energy consumption costmaps to $c_2 = 0.35$, $c_3 = 0.4$ and $c_4 = 0.1$ respectively, while we set the overall thresholding value for the final decision map to $0.7$. For the hierarchical clustering parameters, we choose $0.5\meter$ for the euclidean distance (frame size of UAV being $0.26\meter$) and the depth threshold as $0.05\meter$. The effect of noisy depth data can also be seen in the other costmaps due to which the final decision map does not appear as clear as in the simulation environment. Nevertheless, our landing site search algorithm demonstrates detection of safe landing sites reliably even in situations where an expert safety operator is unable to make decisions. \looseness=-1
